Learning from Video and Text via Large-Scale Discriminative Clustering

Discriminative clustering has been successfully applied to a number of weakly-supervised learning tasks. Such applications include person and action recognition, text-to-video alignment, object co-segmentation and colocalization in videos and images. One drawback of discriminative clustering, however, is its limited scalability. We address this issue and propose an online optimization algorithm based on the Block-Coordinate Frank-Wolfe algorithm. We apply the proposed method to the problem of weakly supervised learning of actions and actors from movies together with corresponding movie scripts. The scaling up of the learning problem to 66 feature length movies enables us to significantly improve weakly supervised action recognition.

==> optimization.tex <==
%%%%%%%%%%%%%%%%%%%%
%%% OPTIMIZATION %%%
%%%%%%%%%%%%%%%%%%%%

\section{Optimization}
\label{sec:optim}

For both problems~\eqref{eq:finalproblem} and~\eqref{eq:finalproblemaction}, we consider a simple continuous convex relaxation and add slack
variables to the constraints~\eqref{eq:one-constraint} and~\eqref{eq:person-action-constraint} (more details in Supplementary Material).
% We replace binary latent variables $Z$ and $T$ by continuous ones that take values in $[0,1]^{N \times P}$ and $[0, 1]^{M \times A}$ respectively.

We can solve the person recognition optimization problem~\eqref{eq:finalproblem} independently on each movie using any standard QP solver\footnote{For instance using the MOSEK toolbox: https://www.mosek.com/}.
For the action recognition problem, we need to optimize jointly over all the movies as action classes are shared.
%As mentionned in the previous section, Prob.~\eqref{eq:finalproblemaction} is a \hl{***}-dimensional quadratic problem.
% you never talk about kernels...
% First, the total number of body tracks $M$ grows linearly with the number of movies.
% $M$ can thus reach values for which it becomes not tractable to use kernelized version of DIFFRAC. 
% In fact, we would need to store a $\mathbb{R}^{M \times M}$ matrix in memory.
% To address this issue, we instead use the linear formulation of DIFFRAC \cite{bach07diffrac}.
First, storing the $M \times M$ matrix $B$~\eqref{eq:finalproblemaction} in memory is prohibitive when the total number of person tracks $M$ is high (\ie it represents more than 100GB when $M \geq 200000$).
Second, batch optimization techniques require to do a full pass over the data in order to perform an update hence having a time complexity of order at least $M$.
To overcome these two issues, we develop a new technique to solve the discriminative clustering objective with constraints based on the online Block-Coordinate variant of the Frank-Wolfe (BCFW) algorithm~\cite{lacoste13bcfw}.

\subsection{Block-coordinate Frank-Wolfe}
\label{sec:BCFW}

%%When dealing with optimization problem of the form $\min_{T\in\mathcal{T}} f(T)$, where the convex feasible set $\mathcal{T}$ is compact and the function $f$ is convex, the Frank-Wolfe algorithm~\cite{frank56algorithm} is an iterative optimization procedure that only requires to optimize \emph{linear} functions over $\mathcal{T}$.
%%Each step of the algorithm consists in computing the gradient at the current iterate in order to obtain a \emph{linear} approximation of the function.
%%This approximation is then minimized on the set $\mathcal{T}$, and the solution is used to get the direction for the next update.
The Block-Coordinate version of the Frank-Wolfe algorithm~\cite{lacoste13bcfw} is used when the convex feasible set $\mathcal{T}$ can be written as a Cartesian product of $n$ smaller sets of constraints: $\mathcal{T}=\mathcal{T}^{(1)}\times\ldots\times \mathcal{T}^{(n)}$.
Inspired by coordinate descent techniques, BCFW consists of updating one variable block $\mathcal{T}^{(i)}$ at a time with a reduced Frank-Wolfe step.
This method has potentially $n$ times cheaper iterates both in space and time.

%%It can be provably up to $n$ times faster while preserving the different appealing properties of the Frank-Wolfe algorithm: (i) explicit \emph{optimal} step size for quadratic objectives, (ii) free \emph{duality gap} computation which can be used as a stopping criterion and (iii) only requires a \emph{linear} oracle.

\paragraph{Movie decomposition.} 
We observe that the set of constraints $\mathcal{T}$ of problem~\eqref{eq:finalproblemaction} naturally decompose over the different movies.
Two bags from different movies cannot indeed share a same track.
The global variable $T\in\mathcal{T}^{(1)}\times\ldots\times \mathcal{T}^{(n)}$ is simply obtained by concatenating the individual action assignment matrices $(T^{(1)},\ldots,T^{(n)})$ corresponding to the $n$ movies.
We can therefore apply the BCFW algorithm for our problem.
%As the challenging part lies in the action assignment variable $T$ and for the sake of simplicity, we omit in the following the slack variable $\xi$.
%However, everything we discuss now can be straighforwardly applied with slack variables as explained in the Appendix.

\subsection{BCFW for DIFFRAC}
In order to use the BCFW method efficiently, we have to ensure that the time and space complexity of a block update does not depend on the total size $M$ of the problem (here number of tracks) but rather depends on the size $M_i$ of the smaller block $i$.
While it was shown to be possible for the structured SVM~\cite{lacoste13bcfw}, it does not necessarily follows for another problem.
After a block is sampled, the update consists of two steps.
First, the gradient with respect to the block is computed. 
Then the \emph{linear oracle} is called to obtain the next iterate.
As we show now, the difficult part in our case is to efficiently compute the gradient with respect to the block.

\paragraph{Block gradient: a naive approach.} 
Let's denote $M_{i}$ the number of tracks for movie $i$.
The objective function $f$ of problem~\eqref{eq:finalproblemaction} is $f(T)= \langle T, B(X,\mu) T\rangle_{\mathrm F} $, where
\begin{equation}
  B(X,\mu) = \frac{1}{M} (I_{M} - X(X^\top X + M \mu I_{d})^{-1}X^\top).
\end{equation}
In order to efficiently compute the block gradients, one can precompute the matrix $P=(X^\top X + M\mu I_{d})^{-1}X^\top\in\mathbb{R}^{d\times M}$.
We can write the block gradient with respect to movie $i$ as follows:
\begin{equation}
\label{eq:block-gradient}
\nabla_{(i)}f(T) = \frac{2}{M} (T^{(i)} - X^{(i)}PT),
\end{equation}
where $T^{(i)} \in \mathbb{R}^{M_{i}\times A}$ and $X^{(i)}\in \mathbb{R}^{M_{i}\times d}$ are respectively the action assignment variable and the feature matrix of movie $i$.
The first interesting fact is that we avoid storing the $B$ matrix. However,
because of the $PT$ matrix multiplication, naively computing this formula has the complexity $\mathcal{O}(MdA)$, where $M$ is the number of body tracks computed across all movies, $d$ the dimensionality of the feature space and $A$ the number of actions.
As this still depends linearly on $M$, we need to find a better way to compute the block gradients, which we describe next.

\paragraph{Block gradient: a smart update.} 
We now propose an update rule with time and space complexity depending on $M_{i}$ instead of $M$ for each iteration by avoiding the re-computation of the block gradients. 
The main intuition is that we need to find a way to store information about all the blocks in a compact form.
A natural way of doing that is to maintain the weights of the linear regression parameters $W \in \mathbb{R}^{d\times A}$.
From~\eqref{eq:W}, we have that $W = PT$.
If we are able to maintain the variable $W$ at each iteration with the desired complexity $\mathcal{O}(M_idA)$, then the block gradient computation~\eqref{eq:block-gradient} can be reduced from $\mathcal{O}(MdA)$ to $\mathcal{O}(M_idA)$.
We now explain how to effectively do it.

At each iteration $t$ of the algorithm, we only update a block $i$ of $T$ while keeping all other blocks fixed.
By denoting $D_t\in\mathbb{R}^{M\times A}$ the direction of update and  $\gamma_t$ the step size, the update becomes
\begin{equation}
\label{eq:block-update}
T_{t+1} = T_t + \gamma_t D_t.
\end{equation}
Therefore, the update rule for the weight variable $W_t$ is as follows:
\begin{equation}
\begin{split}
\label{eq:weight-update}
&W_{t+1} = P(T_t + \gamma_t D_t) \\
&W_{t+1} = W_{t} + \gamma_{t} PD_t \\
&W_{t+1} = W_{t} + \gamma_{t} P^{(i)}D_t^{(i)} 
\end{split}
\end{equation}
where  $P^{(i)}$ and $D_t^{(i)}$ are respectively the i-th horizontal blocks of matrix $P$ and $D_t$ with $P^{(i)} \in \mathbb{R}^{d\times M_{i}}$ and $D_t^{(i)}\in  \mathbb{R}^{M_{i}\times A}$.
The first equality in~\eqref{eq:weight-update} follows from the definition of $W$ and the third equality comes from the fact that the  direction of update has non zero value only inside block $i$.
The computational complexity of the update of $W$ is in $\mathcal{O}(M_{i}dA)$ which is what we wanted.

%\paragraph{Approximate gap sampling and line-search.}
%The block gaps can be used to perform adaptive sampling of the blocks~\cite{osokin16bcfw} in order to speed-up convergence.
%We follow this method in our work.
%The block gap can be computed cheaply as follows:
%\begin{equation}
%\label{eq:gap}
% g_i^{(t)}  =  \langle D^{(i)}_t , \nabla_{(i)}f(T_{t})\rangle_{\mathrm F} 
%\end{equation}
%Thanks to the quadratic objective, we can find the optimal step size in closed form (see Algorithm~\ref{CHalgorithm}).

We managed to design a Block-Coordinate Frank-Wolfe update with a time and space complexity which only depends on the block sizes. 
Thus, the BCFW method can be effectively used.
This allows to scale our problem to an arbitrary large number of movies and tracks.
The pseudo-code of the algorithm is given in Algorithm~\ref{CHalgorithm}.

\definecolor{comment}{RGB}{86, 115, 154}

\begin{algorithm}[t!]
\caption{BCFW for DIFFRAC}
\label{CHalgorithm}
\begin{algorithmic}
\State Initiate $T_0$, $P:=(X^\top X + M\mu I_{d})^{-1}X^\top$, $W_0=PT_0$, $g_i=+\infty, \ \forall i$.
\For{ $t$ in 0:$N_{iter}$}
\State $i$ $\gets$ sample from distribution proportional to $\textit{g}$ \cite{osokin16bcfw}
\State {\color{comment} \footnotesize \# Block gradient computation}
\State $\nabla_{(i)}f(T_t)$ $\gets$ $\frac{2}{M}(T^{(i)}_t - X^{(i)}W_t)$  
\State {\color{comment} \footnotesize \# Linear oracle computation}
\State $T_{min}$ $\gets$ $\argmin_{y \in \mathcal{T}^(i)} \langle \nabla_{(i)}f(T_t), y\rangle_{\mathrm F}$ 
\State {\color{comment} \footnotesize \# Block gap and line-search computation}
\State $D \gets T^{(i)} - T_{min} $
\State $g_i \gets \langle D, \nabla_{(i)}f(T_t)\rangle_{\mathrm F}$ 
\State $ \gamma \gets \min(1,\frac{g_i}{\frac{2}{M} \langle D, D-X^{(i)}P^{(i)}D\rangle_{\mathrm F}}) $ 
\State {\color{comment} \footnotesize \# W update}
\State $W_{t+1}$ $\gets$  $W_t - \gamma P^{(i)}D$
\State {\color{comment} \footnotesize \# Block update}
\State $T^{(i)}_{t+1} \gets T_t^{(i)} - \gamma D$
\EndFor
\end{algorithmic}
\end{algorithm}


%\paragraph{Rounding.}
%One natural way to round $Z$ (or $T$) is to consider the latent variables resulting from the previous optimization problem. 
%Then we compute the orthogonal projection according to the \(\mathcal{L}_2\) norm on this following binary matrices set \(\mathcal{Z} = \{Z \in \{0,1\}^{N \times P} \ | \ Z \mathbf{1}_P = \mathbf{1}_N\}\)
%\begin{align}
%  \arg \min_{\hat{Z} \in \mathcal{Z}} \|\hat{Z} - Z_{min}\|_2.
%\end{align}
%It is equivalent to taking the maximum value of each line of $Z$. 
%\cite{bojanowski15weakly} proposed to do it by retrieving the ridge regression parameters $W$ that was trained on the latent variables $Z_{min}$. 
%Instead of projecting $Z_{min}$ on $\mathcal{Z}$, we can project $XW$ on $\mathcal{Z}$. 
%It can be written formally as:
%\begin{align}
%   \arg \min_{\hat{Z} \in \mathcal{Z}} \|\hat{Z} - X_{1}(X_{1}^TX_{1}+N\lambda I_{N})^{-1}X_{1}^T Z_{min}\|_2.
%\end{align}

%\subsection{Discussion}
%\hl{JB: Don't know if we need the discussion session???}
%\hl{Piotr: I think we do as this is the main claim of the paper...}



